Embedding Symbolic Knowledge into Deep Networks

In this work, we aim to leverage prior symbolic knowledge to improve the performance of deep models. We propose a graph embedding network that projects propositional formulae (and assignments) onto a manifold via an augmented Graph Convolutional Network (GCN). To generate semantically-faithful embeddings, we develop techniques to recognize node heterogeneity, and semantic regularization that incorporate structural constraints into the embedding. Experiments show that our approach improves the performance of models trained to perform entailment checking and visual relation prediction. Interestingly, we observe a connection between the tractability of the propositional theory representation and the ease of embedding. Future exploration of this connection may elucidate the relationship between knowledge compilation and vector representation learning.

==> discussion.tex <==
\section{Discussion: Extensions \& Future Work}
\label{sec-discussion}
% what can it be used for?

%The results in the previous sections show that LENSeR learns informative logic embeddings, which can be used to improve a target model on the real-world task of VRP. Overall, our results suggest that constraining embeddings to be semantically faithful, e.g., by allowing for node heterogeneity and through regularization, aids model training.

==> experiments-nlp.tex <==
%\section{Natural Language Translation}
We further extend our model beyond propositional logic to more general rule. We applied our framework to Neural Machine Translation (NMT) domain by incorporating grammar rules. 

\textbf{Model}
Instead of logic formulas, we extend our embedder to Context Free Grammar (CFG), which is a certain type of formal grammar with a set of production rules that describe all possible strings in a given formal language. Production rules are simple replacements. These rules can be applied regardless of context. All rules are one-to-one, one-to-many, or one-to-none, i.e. the left-hand side of the production rule is always one nonterminal symbol and the right handside could be one or more nonterminal or terminal symbol, where the nonterminal symbol does not appear in the resulting formal language. 
In the CFG graph, nodes are nonterminal symbols, terminal symbols, IMPLY operator, AND operator and Global node. The left handside connects to the respective IMPLY operator, The right handside components will connect to an AND operator node first, then this AND node and the IMPLY node will be connected. Besides, the adjacent words are connected in the sentence graph, i.e. truth assignment graph. 
Using the dataset and graph creation method, we tested the performance of different embedders and the baseline (w/o embedding loss).


\textbf{Dataset}
We use IWSLT'14 German to English (De-En) translation task dataset \cite{Cettolo2014}. We on purposely choose the target language to be English such that the grammar rules are easier to obtain. We use a similar setup of \cite{EdunovOAGR18} for 160K training sentence pairs, 7K validation sentences pairs and the test set is the concatenation of all available test and dev sets of IWSLT 2014 which is of similar sie to the validation set.
%, that is TED.tst2010, TED.tst2011, TED.tst2012 and TED.dev2010, TEDX.dev2012 which is of similar size to the validation set. 
All data is lower-cased, however, we didn't use byte-pair encoding (BPE) \cite{SennrichHB16a} vocabulary in this work since it's difficult to associate grammar rules with BPE vocabulary although it hurts the translation performance as expected. The evaluation are based on beam search with a beam width of 5, and case-sensitive BLEU4 scores are reported.

\textbf{Implementation Details}
We use the \textit{fairseq-py} toolkit to implement our translation model and embedded with our embedder. Our translation models have XX layers of encoder and XX layers of decoder layer. We use 50d Glove word vector embedding. We use a learning rate of 0.25 and momentum of 0.99.

\textbf{Results}
We compared the results of baseline translation model (no embedder), translation model with standard CFG embedder, directed CFG embedder, heterogeneous CFG embedder and directed-heterogeneous embedder. The results are summarized in Table~\ref{tbl:nlp}. The directed graph variation makes hurts the performance due to the restricted information flow as mentioned above. Furthermore, independent weights didn't improve the performance either. 

\begin{table}
    \label{tbl:nlp}
	\caption{Performance of machine translation w/ or w/o logic embedding loss.}
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		Model & HE & Directed & BLEU \\ \hline
		w/o CFG & - & - &  28.55\\ \hline
		\multirow{4}{*}{CFG} & N & N & \textbf{28.76} \\  
		& N & Y  & 28.42 \\  
		& Y & N  & 28.58 \\  
		& Y & Y  & 28.57 \\ \toprule
	\end{tabular}
\end{table}



%%%%% remove from IJCAI
More broadly, this idea may extend beyond learning logic embeddings. In other words,  LENSeR could be adapted to embed other forms of symbolic knowledge expressible as graph structures. For example, we have applied our general approach to Neural Machine Translation (NMT) by embedding Context Free Grammars (CFGs). Preliminary results (shown in Table~\ref{tbl:nlp} and Fig.~\ref{fig:sentence}) show that a target model trained with LENSeR is able to generate more grammatically compliant and semantically-sound sentences on the IWSLT'14 German to English (De-En) translation task~\cite{Cettolo2014}. Likewise, LENSeR could also be extended to embed temporal logic, which has many applications, including video grounding, dialogue generation, and policy generation. Future work could explore alternative forms of enabling node heterogeneity and semantic regularization for these different forms of prior knowledge.

The gains demonstrated in experiments also suggest a relationship between tractability of a logical form and amenability to embedding. This opens up several directions for future research. First, a theoretical study to understand complexity of embedding from the lens of tractability has potential to yield interesting results. Furthermore, an extensive empirical analysis is warranted given the abundance of  several logical forms discovered over the past two decades with varying degrees of tractability~\cite{Darwiche2002}.

%Since our framework LENSeR is model-agnostic, it's potentially able to incorporate any general symbolic knowledge to enhance the target non-symbolic models. We focus on propositional logic in this work, while it could be easily extend to more general domains. Here are some possible extensions. 
%
%\textbf{Context Free Grammar in Natural Language} \quad
%We further extend our model beyond propositional logic to Context Free Grammar (CFG) and applied LENSeR to Neural Machine Translation (NMT) domain.
%Context Free Grammar (CFG) is a certain type of formal grammar with a set of production rules that describe all possible strings in a given formal language. Production rules are simple replacements. These rules can be applied regardless of context. All rules are one-to-one, one-to-many, or one-to-none, i.e. the left-hand side of the production rule is always one nonterminal symbol and the right handside could be one or more nonterminal or terminal symbol, where the nonterminal symbol does not appear in the resulting formal language. 
%In the CFG graph, nodes are nonterminal symbols, terminal symbols, IMPLY operator, AND operator and Global node. The left handside connects to the respective IMPLY operator, The right handside components will connect to an AND operator node first, then this AND node and the IMPLY node will be connected. Besides, the adjacent words are connected in the sentence graph, i.e. truth assignment graph. 
%Using the dataset and graph creation method, we tested the performance of different embedders and the baseline (w/o embedding loss).
%
%We use IWSLT'14 German to English (De-En) translation task dataset \cite{Cettolo2014}. We on purposely choose the target language to be English such that the grammar rules are easier to obtain. We use a similar setup of \cite{EdunovOAGR18} for 160K training sentence pairs, 6,750 validation sentences pairs and the test set is the concatenation of all available test and dev sets of IWSLT 2014 which is of similar size to the validation set.
%However, as a preliminary experiment, we didn't use byte-pair encoding (BPE) \cite{SennrichHB16a} vocabulary in this work since it's difficult to associate grammar rules with BPE vocabulary, which hurts the translation performance as expected. 
%
%The evaluation are based on beam search with a beam width of 5, and case-sensitive BLEU4 scores are reported. Since BLEU scores are not appropriate to measure grammar correctness~\cite{Sulem2018,napoles2016}, we also report reference-less metric, which uses grammatical error detection tools. In this work we use LT~\cite{Milkowski2010}, the best performing non-proprietary grammaticality metric~\cite{napoles2016}. The LT score of the sentence is defined to be $1-\frac{\textrm{\#errors}}{\textrm{\#tokens}}$, which is the higher the better. The percentages of sentences with errors are also reported as ``sentence-level error rate''. 
%
%We are able to improve the machine translation performance with grammar rules as shown in Table~\ref{tbl:nlp}. Generated sentence examples, as shown in Figure~\ref{fig:sentence}, illustrated that model trained with LENSeR is able to generate more grammatically complied and semantically sound sentences. Future work is needed to improve further, such as BPE vocabulary grammar, hyper-parameters tuning, finer grammar selection. The preliminary experiments demonstrate the potential of LENSeR to boost other natural language processing tasks by considering symbolic knowledge.

\begin{table}
\centering
    \caption{Performance of machine translation w/ or w/o CFG measured by BLEU, LT~\protect\cite{Milkowski2010}, and SER (sentence-level error rate). The best scores are in bold.}
	\begin{tabular}{c|c|c|c}
		\toprule
		Model  & BLEU & LT & SER (\%)\\ \specialrule{0.8pt}{1pt}{1pt}
		w/o CFG &  28.55 & 0.9821 & 20.28 \\ \hline
		w/ CFG & \textbf{28.78}& \textbf{0.9860} & \textbf{17.13} \\ 
		\bottomrule
	\end{tabular}
\label{tbl:nlp}
\end{table}

\begin{figure}
\centerline{\includegraphics[page=8,width=0.45\textwidth]{figures/analysis}}
\caption{Generated sentences examples. Incorrect grammars are highlighted in red and the corresponding generations by the other model are in green. Our LENSeR is able to encourage the generation of grammatically correct sentences by incorporation grammar rules.}
\label{fig:sentence}
\end{figure}


%LENSeR could be also be extended to embed temporal logic. Temporal logic has vast applications, such as video grounding, chat bots and robotics. For example, in video grounding where the task is to ground the activities and scenes in the video, common sense rules could be used to regulate the activities grounding, e.g. you need to pick up the banana before peeling it. Incorporating temporal logic in real world tasks is a useful and promising further direction. 



==> experiments.tex <==
% \section{Experiments}
% \subsection{Experimental Setup}
% % This is a incremental setup, synthetic propositional logic -> real problem propositional logic -> general logic (CFG) (less constrained)

% task + dataset + model

\input{experiments-synthetic.tex}
\input{experiments-vrd.tex}

\section{Natural Language Translation}
We further extend our model beyond propositional logic to more general rule. We applied our framework to Neural Machine Translation (NMT) domain by incorporating grammar rules. 

\textbf{Model}
Instead of logic formulas, we extend our embedder to Context Free Grammar (CFG), which is a certain type of formal grammar with a set of production rules that describe all possible strings in a given formal language. Production rules are simple replacements. These rules can be applied regardless of context. All rules are one-to-one, one-to-many, or one-to-none, i.e. the left-hand side of the production rule is always one nonterminal symbol and the right handside could be one or more nonterminal or terminal symbol, where the nonterminal symbol does not appear in the resulting formal language. 
In the CFG graph, nodes are nonterminal symbols, terminal symbols, IMPLY operator, AND operator and Global node. The left handside connects to the respective IMPLY operator, The right handside components will connect to an AND operator node first, then this AND node and the IMPLY node will be connected. Besides, the adjacent words are connected in the sentence graph, i.e. truth assignment graph. 
Using the dataset and graph creation method, we tested the performance of different embedders and the baseline (w/o embedding loss).


\textbf{Dataset}
We use IWSLT'14 German to English (De-En) translation task dataset \cite{Cettolo2014}. We on purposely choose the target language to be English such that the grammar rules are easier to obtain. We use a similar setup of \cite{EdunovOAGR18} for 160K training sentence pairs, 7K validation sentences pairs and the test set is the concatenation of all available test and dev sets of IWSLT 2014 which is of similar sie to the validation set.
%, that is TED.tst2010, TED.tst2011, TED.tst2012 and TED.dev2010, TEDX.dev2012 which is of similar size to the validation set. 
All data is lower-cased, however, we didn't use byte-pair encoding (BPE) \cite{SennrichHB16a} vocabulary in this work since it's difficult to associate grammar rules with BPE vocabulary although it hurts the translation performance as expected. The evaluation are based on beam search with a beam width of 5, and case-sensitive BLEU4 scores are reported.

\textbf{Implementation Details}
We use the \textit{fairseq-py} toolkit to implement our translation model and embedded with our embedder. Our translation models have XX layers of encoder and XX layers of decoder layer. We use 50d Glove word vector embedding. We use a learning rate of 0.25 and momentum of 0.99.

\textbf{Results}
We compared the results of baseline translation model (no embedder), translation model with standard CFG embedder, directed CFG embedder, heterogeneous CFG embedder and directed-heterogeneous embedder. The results are summarized in Table~\ref{tbl:nlp}. The directed graph variation makes hurts the performance due to the restricted information flow as mentioned above. Furthermore, independent weights didn't improve the performance either. 

\begin{table}[]
\centering
	\caption{Performance of machine translation w/ or w/o logic embedding loss.}
	\begin{tabular}{c|c|c|c}
		\toprule
		Model & HE & Directed & BLEU \\ \hline
		w/o CFG & - & - &  28.55\\ \hline
		\multirow{4}{*}{CFG} & N & N & \textbf{28.76} \\  
		& N & Y  & 28.42 \\  
		& Y & N  & 28.58 \\  
		& Y & Y  & 28.57 \\ \toprule
	\end{tabular}
\label{tbl:nlp}
\end{table}
